Joint Event Detection and Entity Resolution: a Virtuous Cycle

Clustering web documents has numerous applications, such as aggregating news articles into meaningful events, detecting trends and hot topics on the Web, preserving diversity in search results, etc. At the same time, the importance of named entities and, in particular, the ability to recognize them and to solve the associated co-reference resolution problem are widely recognized as key enabling factors when mining, aggregating and comparing content on the Web. Instead of considering these two problems separately, we propose in this paper a method that tackles jointly the problem of clustering news articles into events and cross-document co-reference resolution of named entities. The co-occurrence of named entities in the same clusters is used as an additional signal to decide whether two referents should be merged into one entity. These refined entities can in turn be used as enhanced features to re-cluster the documents and then be refined again, entering into a virtuous cycle that improves simultaneously the performances of both tasks. We implemented a prototype system and report results using the TDT5 collection of news articles, demonstrating the potential of our approach.

==> feedback.tex <==
The fact alone of improving the named entity co-reference by refining the output of the parser may already be interesting enough in many applications.
But as the named entities were also used for the clustering any improvement on their co-reference should repercute on the clustering. 
This is, for each equivalence class obtained in the previous section we create a new entity that aggregates the occurrences of all entities in the class.
The original entities are removed, and the clustering can then be relaunched.
This process can then be repeated by re-analyzing which named entities to merge and re-cluster for a third time.
However in the co-reference module it has now to be specified how to compare two potential equivalence class of entities.
For the social similarity threshold this is straightforward, as we said that the occurrence vector of the new representative entity is the union of the occurrences of all the expression in the class it represents.
With respect to the content features the issue is not as trivial, because several -- eventually incompatible -- expressions where merged.
We decided to take the maximal similarity between the members of the two classes. 
This is, if $N_1$ is the representative of the class $\langle n^{(1)}_1 \dots n^{(1)}_i \rangle$ and $N_2$ of $\langle n^{(2)}_1 \dots n^{(2)}_j \rangle$, then $\text{sim}(N_1, N_2) = \max_{n_1 \in N_1, n_2 \in N_2} \text{sim}(n_1,n_2)$. 
This is consistent with our decision of taking the transitive closure in the previous section, and corresponds to the simple-link version of a hierarchical agglomerative clustering.



